Retrieval augmentation of large language models for lay language generation

Recent lay language generation systems have used Transformer models trained on a parallel corpus to increase health information accessibility. However, the applicability of these models is constrained by the limited size and topical breadth of available corpora. We introduce CELLS, the largest (63k pairs) and broadest-ranging (12 journals) parallel corpus for lay language generation. The abstract and the corresponding lay language summary are written by domain experts, assuring the quality of our dataset. Furthermore, qualitative evaluation of expert-authored plain language summaries has revealed background explanation as a key strategy to increase accessibility. Such explanation is challenging for neural models to generate because it goes beyond simplification by adding content absent from the source. We derive two specialized paired corpora from CELLS to address key challenges in lay language generation: generating background explanations and simplifying the original abstract. We adopt retrieval-augmented models as an intuitive fit for the task of background explanation generation, and show improvements in summary quality and simplicity while maintaining factual correctness. Taken together, this work presents the first comprehensive study of background explanation for lay language generation, paving the path for disseminating scientific knowledge to a broader audience. CELLS is publicly available at: https://github.com/LinguisticAnomalies/pls_retrieval.

==> tables/case_study.tex <==
\begin{table*}[]
\centering

\begin{tabular}{@{}m{1.5cm}<{}m{14cm}<{}@{}}
\toprule
\textbf{Model}       & \textbf{Text} \\
\midrule
Source  & When incorporated into a polypeptide chain, proline (Pro) differs from all other naturally occurring amino acid residues in two important respects. The ph dihedral angle of Pro is constrained to values close to -65deg and Pro lacks an amide hydrogen.\\
\midrule
Target  & Unlike other amino acids that constitute proteins, Proline is missing a vital hydrogen atom and also bestows local structural rigidity to the three-dimensional ( 3D) structure of proteins.\\
\midrule
BART        & Proline ( Pro) is a naturally occurring amino acid residue in \textcolor{violet}{the human genome that plays an important role in the regulation of gene expression.}\\
\midrule
BART-Pubmed & The ph dihedral angle of proline ( Pro) is constrained to values close to -65deg and Pro lacks an amide hydrogen.\\
\midrule
BART-UMLS   & The amino acid proline ( Pro) is \textcolor{teal}{the most abundant} naturally occurring amino acid \textcolor{brown}{in eukaryotic cells} and \textcolor{violet}{plays an important role in the regulation of protein synthesis}. \\
\midrule
BART-Wiki   & The amino acid proline ( Pro) is \textcolor{teal}{the most abundant} naturally occurring amino acid  \textcolor{brown}{in eukaryotic proteins} and \textcolor{violet}{plays an important role in protein structure and function}.\\
\midrule
BART-RAG & Proline ( Pro) is one of \textcolor{the most abundant} naturally occurring amino acids \textcolor{brown}{in eukaryotes} and \textcolor{violet}{plays an important role in protein folding and protein-protein interactions}. Proline is unique among all other amino acid residues in two important respects: 1) its dihedral angle is close to -65deg and 2) it lacks an amide hydrogen, \textcolor{blue}{which makes it difficult to use it as a template for protein engineering}. \\
\bottomrule
\end{tabular}
\caption{Example of generated texts. External contents that are not available in the source are highlighted. Contents with similar meanings are highlighted using same color. }
\label{case}
\end{table*}

==> tables/dataset_description.tex <==
\begin{table*}
%\small
\centering
% \begin{tabular}{m{1.5cm}<{}|m{0.8cm}<{\centering}m{0.8cm}<{\centering}|m{0.8cm}<{\centering}m{0.8cm}<{\centering}|m{0.8cm}<{\centering}m{0.8cm}<{\centering}}
\begin{tabular}{@{} l rr rr rr@{}}
\toprule
% \multicolumn{1}{|c|}{\multirow{2}{*}{Statistic}} 
% & \multicolumn{2}{c}{\bf Train}  \\ 
% \cmidrule(lr){2-3}
& \multicolumn{2}{c}{\textbf{Paragraph}} & \multicolumn{2}{c}{\textbf{Background}} & \multicolumn{2}{c}{\textbf{Sentence}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
& \textbf{Source}  & \textbf{Target} & \textbf{Source}  & \textbf{Target}& \textbf{Source}  & \textbf{Target}\\     
\midrule
Numbers                     & 62,886  & 62,886  & 47,157 & 47,157 & 233,916 & 233,916 \\
Average length (words)      & 284     & 178     & 52     & 57     & 28      & 27      \\
Vocabulary size             & 315,570 & 171,477 & 90,221 & 64,205 & 177,695 & 130,824 \\
\midrule
Flesch-Kincaid              & 15.16   & 15.03*  & 15.52  & 14.81*  & 15.88   & 15.17*   \\
Coleman-Liau                & 16.61   & 16.41*  & 17.57  & 16.66*  & 16.73   & 16.05*   \\
Automated Readability Index & 18.12   & 17.84*  & 18.55  & 17.61*  & 18.93   & 18.03*   \\
\bottomrule

\end{tabular}
\caption{Dataset lexical feature statistics. * indicates statistical significant difference in paired t-test with $p-value < 0.05$.}
\label{data_description}

\end{table*}

==> tables/difficulty.tex <==
\begin{table}[]
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{} lccccccccc@{}}
% \begin{tabular}{p{0.15\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth}}
\toprule
\textbf{Models}     & \textbf{Verb}     & \textbf{Noun}     & \textbf{Num}  & \textbf{Length} \\
\midrule
Source     & 12.25 & 32.97 & 0.91 & 51.98 \\
Target     & 12.79 & 32.13 & 0.75 & 47.01 \\
\midrule
BART        & 11.74 & 33.79 & 0.73 & 29.41 \\
BART-PubMed & 11.84 & 33.51 & 0.70 & 30.38 \\
BART-UMLS   & 11.94 & 33.75 & 0.72 & 29.06 \\
BART-Wiki   & 12.00 & 33.73 & \textbf{0.64} & 29.41\\
BART-RAG   & \textbf{12.26} & \textbf{32.81} & 0.79 & 38.51\\
\bottomrule
\end{tabular}
% %
% }

\caption{The percentage of nouns, verbs and numbers and the average length of the source, target and models' generated texts. Simple text contains more verbs, fewer nouns and fewer numbers.}
\label{tab:difficulty}
\end{table}


% \begin{table*}[]
% \centering
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{} lccccccccc@{}}
% % \begin{tabular}{p{0.15\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth} p{0.05\linewidth}}
% \toprule
% \textbf{Models}     & \textbf{Verb}     & \textbf{Noun}     & \textbf{Num}  & \textbf{Length}   & \textbf{Flesch}    & \textbf{Coleman}  & \textbf{Auto}  & \textbf{PS} & \textbf{WF}\\
% \midrule
% Source     & 12.25 & 32.97 & 0.91 & 51.98 & 15.59 & 17.58 & 18.62 & 0.23           & 4.04            \\
% Target     & 12.79 & 32.13 & 0.75 & 47.01 & 14.89 & 16.68 & 17.71 & 0.78           & 3.77            \\
% \midrule
% BART        & 11.74 & 33.79 & 0.73 & 29.41 & 15.38 & 16.53 & 18.51 & 0.76           & 3.93            \\
% BART-PubMed & 11.84 & 33.51 & 0.70 & 30.38 & 15.47 & 16.53 & 18.49 & 0.77           & 3.91            \\
% BART-UMLS   & 11.94 & 33.75 & 0.72 & 29.06 & \textbf{15.10} & 16.40 & \textbf{18.08} & 0.76           & 3.89            \\
% BART-Wiki   & 12.00 & 33.73 & \textbf{0.64} & 29.41 & 15.50 & 16.65 & 18.57 & 0.76           & 3.93            \\
% BART-RAG   & \textbf{12.26} & \textbf{32.81} & 0.79 & 38.51 & 15.18 & \textbf{16.10} & 18.18 & \textbf{0.79}           & \textbf{3.80}           \\
% \bottomrule
% \end{tabular}
% % %
% % }

% \caption{Text difficulty evaluation for background explanation. Simple text has more verbs and less nouns. Plain language summary usually has less numbers. Length: text length; Flesch: Flesch-Kincaid grade level; Cole: Coleman-Liau index; Auto: Automated readability index; PS: plain score generated by the classification model. Higher score indicates more plain; WF: word familiarity based on Wikipedia inverse document frequency. Lower means more common words.(Best model performance is in blod.)}
% \label{difficulty}
% \end{table*}

==> tables/external_category.tex <==
\begin{table*}[]
\centering
\tiny
\begin{tabular}{@{}m{1.4cm}<{\centering}m{3.55cm}<{\centering}m{3.55cm}<{\centering}m{3.55cm}<{\centering}m{3.55cm}<{\centering} @{}}
\textbf{Category} &\textbf{Source} & \textbf{Target} & \textbf{BART-wiki} & \textbf{BART-rag}   \\
Term definition                      
% & When incorporated into a polypeptide chain, proline (Pro) differs from all other naturally occurring amino acid residues in two important respects.                                                                                     
% & Unlike other amino acids that constitute proteins, Proline is missing a vital hydrogen atom and also bestows local structural rigidity to the three-dimensional ( 3D) structure of proteins.                                                                    
% & The amino acid proline ( Pro) is the most abundant naturally occurring amino acid in eukaryotic proteins and plays an important role in protein structure and function.                              
% & Proline ( Pro) is one of the most abundant naturally occurring amino acids in eukaryotes and plays an important role in protein folding and protein-protein interactions.                                                                                        \\
& Zoonotic disease (ZD) pose a serious threat to human health in low-income countries.                                            
& Zoonoses are diseases transmitted from vertebrate animals to humans. They can cause a variety of symptoms ranging from mild gastrointestinal complaints to debilitating illness and even death. Especially in low-income countries where animals play an important role for many, the burden of these diseases can be substantial. However, there is often little attention for these diseases, thus they remain under-researched and underfunded.                                                                      & Zoonotic disease ( ZD) is a serious threat to human health in low-income countries.                                             & Zoonotic disease ( ZD) is a serious public health problem in low-income countries. It is caused by infection of animals with pathogenic protozoa belonging to the genus Orthopoxvirus, which are transmitted to humans through the bites of infected mosquitoes.  \\
Example                              
& Very little is known about how environmental changes such as increasing temperature affect disease dynamics in the ocean, especially at large spatial scales.                                                                           
& Coral reefs have been decimated over the last several decades. The global decline of reef-building corals is of particular concern. Infectious diseases are thought to be key to this mass coral mortality, and many reef ecologists suspect that anomalously high ocean temperatures contribute to the increased incidence and severity of disease outbreaks. This hypothesis is supported by local observations--for example, that some coral diseases become more prevalent in the summertime--but it has never been tested at large spatial scales or over relatively long periods. 
& Disease dynamics in the ocean are influenced by environmental changes such as increasing temperature, but little is known about how these changes affect disease dynamics over large spatial scales. 
& Disease dynamics in the ocean are affected by environmental changes such as temperature, but very little is known about how these changes affect disease dynamics at large scales.                                                                            \\
% Epidemiology studies                 
% & Zoonotic disease (ZD) pose a serious threat to human health in low-income countries.                                            
% & Zoonoses are diseases transmitted from vertebrate animals to humans. They can cause a variety of symptoms ranging from mild gastrointestinal complaints to debilitating illness and even death. Especially in low-income countries where animals play an important role for many, the burden of these diseases can be substantial. However, there is often little attention for these diseases, thus they remain under-researched and underfunded.                                                                      & Zoonotic disease ( ZD) is a serious threat to human health in low-income countries.                                             & Zoonotic disease ( ZD) is a serious public health problem in low-income countries. It is caused by infection of animals with pathogenic protozoa belonging to the genus Orthopoxvirus, which are transmitted to humans through the bites of infected mosquitoes. \\
Rephrasing to interrogative sentence 
& Just as complex electronic circuits are built from simple Boolean gates, diverse biological functions, including signal transduction, differentiation, and stress response, frequently use biochemical switches as a functional module. 
& How does a cell know what type of cell it is supposed to become? How do external chemical signals change the underlying"state" of the cell? How are response pathways triggered on the application of a stress? Such questions of differentiation, signal transduction, and stress response, while seemingly diverse, all pertain to the storage of state information, or"memory," by biochemical switches.                                                                                                             & Many biological functions, including signal transduction, differentiation, and stress response, frequently use biochemical switches as a functional module.                                         
& Many biological functions, including signal transduction, differentiation, and stress response, frequently use biochemical switches as a functional module.  \\                                                                                                   
\end{tabular}
\caption{}
\label{tab:external_category}
\end{table*}

==> tables/generation_quality.tex <==
\begin{table}[]
\small
\centering
\begin{tabular}{cccc}
\toprule
\textbf{Task}                                                                 & \textbf{Models} & \textbf{RL} & \textbf{BERT} \\
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}
Background\\explanation
\end{tabular}}
 & BART                              & 24.67                             & 87.56                                \\
                                                                                               & BART-PubMed                       & 24.70                             & 87.51                                \\
                                                                                               & BART-UMLS                         & 24.51                             & 87.56                                \\
                                                                                               & BART-Wiki                         & \textbf{24.95}                             & \textbf{87.62}                                \\
                                                                                               & BART-RAG                         & 24.91                             & 87.50                                \\ 
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}
% Sentence\\ generation
Sentence-level \\ simplification
\end{tabular}} & BART                              & 23.09                             & 87.99                                \\
                                                                                               & BART-PubMed                       & 24.49                             & \textbf{88.34}                                \\
                                                                                               & BART-UMLS                         & 24.51                             & 87.55                                \\
                                                                                               & BART-Wiki                         & 24.95                             & 87.61                                \\
                                                                                              & BART-RAG                         & \textbf{25.44}                             & 88.30                                \\
\midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}
Paragraph-level \\ LLG
\end{tabular}}  & BART                              & \textbf{44.05}                             & \textbf{87.45}                                \\
                                                                                              & BART-PubMed                       & 38.83                             & 87.08                              
\\

\bottomrule
\end{tabular}
\caption{Models' performance in text generation. We used F1 score ROUGE-L (RL) and BERTScore (BERT) to evaluate the generation quality of models on background explanation, sentence-level simplification and paragraph-level lay language generation (LLG).}
\label{tab:generation_quality}
\end{table}

==> tables/human_eval.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{@{}l l l l l@{}}
\toprule
            & \textbf{Tgt}  & \textbf{Wiki}  & \textbf{RAG}   &  \\
\midrule
Grammar     & 3.50 & 3.81  & 3.88  &  \\
Understandability  & 2.88 & 3.25  & 2.88  &  \\
Meaning preservation & 2.81 & 2.63  & 3.94* &  \\
Correctness of key information & 3.06 & 3.06  & 3.69* &  \\
Relevant external information    & 3.31 & 2.38* & 3.56  & \\
\bottomrule
\end{tabular}
\caption{Human evaluation resultsl. Higher score means better. * indicates statistically significant with p-value=0.05}
\label{tab:human_eval}
\end{table}
